EffiLearner: Enhancing Efficiency of Generated Code via Self-Optimization

Large language models (LLMs) have shown remarkable progress in code generation, but their generated code often suffers from inefficiency, resulting in longer execution times and higher memory consumption. To address this issue, we propose \textbf{EffiLearner}, a self-optimization framework that utilizes execution overhead profiles to improve the efficiency of LLM-generated code. EffiLearner first generates code using an LLM, then executes it locally to capture execution time and memory usage profiles. These profiles are fed back to the LLM, which then revises the code to reduce overhead. To evaluate the effectiveness of EffiLearner, we conduct extensive experiments on the EffiBench, HumanEval, and MBPP with 16 open-source and 6 closed-source models. Our evaluation results demonstrate that through iterative self-optimization, EffiLearner significantly enhances the efficiency of LLM-generated code. For example, the execution time (ET) of StarCoder2-15B for the EffiBench decreases from 0.93 (s) to 0.12 (s) which reduces 87.1% the execution time requirement compared with the initial code. The total memory usage (TMU) of StarCoder2-15B also decreases from 22.02 (Mb*s) to 2.03 (Mb*s), which decreases 90.8% of total memory consumption during the execution process. The source code of EffiLearner was released in https://github.com/huangd1999/EffiLearner

==> backup_results.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Code efficiency of widely-studied LLMs reported by \xxx.}
    \label{tab:end2end}
    \begin{tabular}{l|rr|rr|rr}
        \toprule
        Model&\textbf{ET (s)}&\textbf{NET}&\textbf{MU (Mb)}&\textbf{NMU}&\textbf{TMU (Mb*s)}&\textbf{NTMU}\\
        \midrule
        \multicolumn{7}{c}{Open-source models}\\
        \midrule
\multirow{2}{*}{OpenCodeInterpreter-1.3B} \\
\\

\multirow{2}{*}{OpenCodeInterpreter-6.7B}&0.34&2.41&36.82&1.00&13.36&1.56\\
&0.28&1.91&38.60&1.00&14.16&1.44\\
\multirow{2}{*}{OpenCodeInterpreter-33B}&0.29&2.10&35.48&1.00&13.06&1.93\\
&0.28&2.00&36.30&1.00&11.54&1.64\\
\midrule
\multirow{2}{*}{DeepSeek-1.3B-Ins}\\
\\
\multirow{2}{*}{deepseek-coder-6.7b-instruct}&0.37&2.60&259.73&7.25&555.18&67.70\\
&0.34&2.37&36.97&1.00&13.66&1.46\\
\multirow{2}{*}{deepseek-coder-33b-instruct}&0.29&2.21&34.53&1.06&14.44&2.91\\
&0.25&1.84&32.67&0.99&8.15&1.55\\
\midrule
% \multirow{2}{*}{CodeFuse-DeepSeek-33B}&0.28&2.03&70.91&2.02&123.76&18.01\\
% &0.28&2.03&49.64&1.45&46.66&7.43\\
\multirow{2}{*}{Phind-CodeLlama-34B-v2}&0.52&3.28&157.16&3.36&337.30&24.44\\
&0.40&2.51&68.27&1.45&65.64&4.86\\
\multirow{2}{*}{CodeLlama-34b-hf}&1.05&7.75&57.57&1.70&94.79&15.65\\
&1.02&7.34&40.62&1.11&52.12&7.02\\
\multirow{2}{*}{CodeLlama-70b-Instruct-hf}&0.52&3.93&109.61&3.57&203.92&54.15\\
&0.47&3.84&26.42&1.00&14.53&6.52\\
\multirow{2}{*}{XwinCoder-34B}&0.77&5.68&49.77&1.49&61.36&12.11\\
&0.69&5.11&52.12&1.47&57.89&9.92\\
\multirow{2}{*}{Artigenz-Coder-DS-6.7B}&0.39&2.75&65.73&1.70&95.65&10.87\\
&0.32&2.30&59.00&1.62&79.67&10.73\\
\multirow{2}{*}{Magicoder-S-DS-6.7B}&0.22&1.59&40.19&1.09&17.58&2.28\\
&0.21&1.50&38.29&1.07&15.27&2.22\\
\multirow{2}{*}{Mistral-7B-codealpaca-lora}&2.36&18.40&28.88&1.00&57.92&24.36\\
&1.45&12.17&27.45&1.03&35.46&17.28\\
\multirow{2}{*}{speechless-starcoder2-15b}&0.93&7.58&26.35&1.00&22.02&10.88\\
&0.12&1.03&27.67&1.01&2.03&1.06\\
\midrule
\multicolumn{7}{c}{Closed-source models}\\
\midrule
\multirow{2}{*}{gpt-3.5-turbo-0301}&0.36&2.50&91.25&2.45&157.50&19.75\\
&0.28&2.01&36.08&0.99&12.43&1.64\\
\multirow{2}{*}{gpt-3.5-turbo-0613}&0.35&2.47&41.72&1.15&35.83&4.71\\
&0.33&2.37&35.49&1.00&13.83&1.94\\
\multirow{2}{*}{gpt-3.5-turbo-1106}&0.28&1.96&36.12&1.01&12.79&1.73\\
&0.26&1.90&34.02&1.00&11.41&1.62\\
\multirow{2}{*}{gpt-4-turbo-preview}&0.27&1.96&33.94&1.00&11.82&1.89\\
&0.25&1.88&33.17&1.00&10.18&1.76\\
\multirow{2}{*}{gpt-4}&0.31&2.19&80.88&2.26&129.91&17.90\\
&0.28&2.06&63.82&1.83&80.74&11.86\\
\multirow{2}{*}{claude-3-haiku}&0.36&2.51&48.33&1.30&52.67&6.73\\
&0.33&2.30&37.37&1.03&17.18&2.37\\
\multirow{2}{*}{claude-3-sonnet}&0.42&2.90&60.46&1.62&82.52&10.12\\
&0.35&2.47&42.31&1.17&28.95&3.76\\
        \bottomrule
    \end{tabular}
\end{table*}

